Fairness-Aware Reinforcement Learning (FAReL): A Framework for Transparent and Balanced Sequential Decision-Making

Equity in real-world sequential decision problems can be enforced using fairness-aware methods. Therefore, we require algorithms that can make suitable and transparent trade-offs between performance and the desired fairness notions. As the desired performance-fairness trade-off is hard to specify a priori, we propose a framework where multiple trade-offs can be explored. Insights provided by the reinforcement learning algorithm regarding the obtainable performance-fairness trade-offs can then guide stakeholders in selecting the most appropriate policy. To capture fairness, we propose an extended Markov decision process, $f$MDP, that explicitly encodes individuals and groups. Given this $f$MDP, we formalise fairness notions in the context of sequential decision problems and formulate a fairness framework that computes fairness measures over time. We evaluate our framework in two scenarios with distinct fairness requirements: job hiring, where strong teams must be composed while treating applicants equally, and fraud detection, where fraudulent transactions must be detected while ensuring the burden on customers is fairly distributed. We show that our framework learns policies that are more fair across multiple scenarios, with only minor loss in performance reward. Moreover, we observe that group and individual fairness notions do not necessarily imply one another, highlighting the benefit of our framework in settings where both fairness types are desired. Finally, we provide guidelines on how to apply this framework across different problem settings.

==> DQN.tex <==
\section{Deep Q-Networks (DQN)}
\label{appendix:dqn}

% \tc{Analogously, the performance reward is normalised with 0 as the cumulative maximum, based on a single-objective agent's performance. Across 10 runs, a DQN agent \citep{Mnih2015} reaches a maximum reward of 46.53243 and 906.0 for the job hiring and fraud detection setting, respectively. Therefore, we normalise the results based on these maxima.}


To establish an empirical upper bound for both scenarios, we consider a single-objective reinforcement learning agent, that will only optimise the performance reward. Using these results, we then normalise the radar plots in this section 
% \cite{Mnih2013, Mnih2015} presented a breakthrough in reinforcement learning, by using deep neural networks as function approximators to learn playing Atari games using the Arcade Learning Environment (ALE) \citep{Bellemare2013}. 
% DQN
% Their deep neural network implementation, called Deep Q-Network (DQN), is trained with a variant of the $Q$-learning algorithm (Algorithm \ref{algorithm:Q_learning}), where the weights of the network are updated using stochastic gradient descent (Algorithm \ref{algorithm:SGD}).



